Dissecting the Interplay of Attention Paths in a Statistical Mechanics Theory of Transformers

Despite the remarkable empirical performance of Transformers, their theoretical understanding remains elusive. Here, we consider a deep multi-head self-attention network, that is closely related to Transformers yet analytically tractable. We develop a statistical mechanics theory of Bayesian learning in this model, deriving exact equations for the network's predictor statistics under the finite-width thermodynamic limit, i.e., $N,P\rightarrow\infty$, $P/N=\mathcal{O}(1)$, where $N$ is the network width and $P$ is the number of training examples. Our theory shows that the predictor statistics are expressed as a sum of independent kernels, each one pairing different 'attention paths', defined as information pathways through different attention heads across layers. The kernels are weighted according to a 'task-relevant kernel combination' mechanism that aligns the total kernel with the task labels. As a consequence, this interplay between attention paths enhances generalization performance. Experiments confirm our findings on both synthetic and real-world sequence classification tasks. Finally, our theory explicitly relates the kernel combination mechanism to properties of the learned weights, allowing for a qualitative transfer of its insights to models trained via gradient descent. As an illustration, we demonstrate an efficient size reduction of the network, by pruning those attention heads that are deemed less relevant by our theory.

==> old_files/supmat_old.tex <==
\appendix

\section{Derivation of the kernel renormalization theory}
\subsection{Model definition}
\label{app:model_definition}
We remind the definition of our transformer model from Sec.~\ref{sec:Model} of the main text. We first expand the bare input $x^{\left(0\right)}\in\mathbb{R}^{N_{0}\times{T}}$ to $x^{\left(1\right)}\in\mathbb{R}^{N_{1}\times{T}}$ by a linear transformation: $x_{i,t}^{\left(1\right)}=\frac{1}{\sqrt{N_{0}}}\sum_{j=1}^{N_{0}}V_{ij}^{\left(0\right)}x_{j,t}^{\left(0\right)}$, where $V^{(0)}_{ij}$ are learnable parameters, $i=1,\ldots,N_{1}$, and  $t=1,\ldots,T$. We can then define the output from each attention layer $ \ell=1,\ldots,L$ recursively:
\begin{equation}
x_{i,t}^{\left(\ell+1\right)}=\frac{1}{\sqrt{N_{\ell}{H}_{\ell}}}\sum_{s=1}^{{T}}\sum_{h=1}^{{H}_{\ell}}\sum_{j=1}^{N_{\ell}}V_{ij}^{\left(\ell\right)h}x_{j,s}^{\left(\ell\right)}\Omega_{st}^{\left(\ell\right)h}\qquad i=1,\ldots,N_{\ell+1}\;,\qquad t=1,\ldots,T\;,
\end{equation}
where $H_\ell$ and $N_\ell$ denote respectively the number of heads and the width of the $\ell$-th layer, while for simplicity in the main text we set $N_\ell=N$, $H_\ell=H$ for each $\ell$. The attention matrix $\Omega^{\left(\ell\right)h}\in\mathbb{R}^{T\times T}$ is defined
as
\begin{equation}
\Omega_{st}^{\left(\ell\right)h}=\zeta\left(\frac{\beta}{N_{0}\sqrt{G}}x_{s}^{\left(0\right)\top}\cdot K^{\left(\ell\right)h}\cdot Q^{\left(\ell\right)h}\cdot x_{t}^{\left(0\right)}\right)\;.
\end{equation}
The function $\zeta$ denotes the softmax applied along the direction of the $s$-th token, while the hyperparameter $\beta$ controls the ``hardness'' of the softmax function. The readout is linear and is parametrized by $a\in\mathbb{R}^{1\times N_{L+1}}$
\begin{equation}
    f=\frac{1}{\sqrt{N_{L+1}}}a\cdot x_{i,t^{*}}^{\left(L+1\right)}\;,
\end{equation}
where we adopt the unified notation
\begin{equation}
    \;\;x_{i,t^{*}}^{\left(L+1\right)}=\begin{cases}
        \frac{1}{T}\sum_{t=1}^Tx_{i,t}^{\left(L+1\right)}&\qquad \text{average over all the tokens}\\\\
\;\;x_{i,1}^{\left(L+1\right)}&\qquad\text{reading from the first token}
\\\\
\;\;x_{i,T}^{\left(L+1\right)}&\qquad\text{reading from the last token}
    \end{cases}\;\;,
\end{equation}
in order to consider different types of tasks. 
\paragraph{Effective description ---} 
It is useful to collect the value matrices into a set of ``effective weights''
\begin{equation}
V^{\left(\mathrm{eff}\right)h_{1}h_{2}\ldots h_{L}}\coloneqq a\cdot V^{\left(L\right)h_{L}}\cdot V^{\left(L-1\right)h_{L-1}}\cdot\ldots\cdot V^{\left(2\right)h_{2}}\cdot V^{\left(1\right)h_{1}}\;.
\end{equation}
We also define the ``attentioned input'' 
\begin{equation}
\xi^{(0)h_{1}h_{2}\ldots h_{L}}\coloneqq\sum_{t_{0},\ldots,t_{L-1}=1}^{T}x_{t_{0}}^{\left(0\right)}\Omega_{t_{0}t_{1}}^{\left(1\right)h_{1}}\Omega_{t_{1}t_{2}}^{\left(2\right)h_{2}}\ldots\Omega_{t_{L-2}t_{L-1}}^{\left(L-1\right)h_{L-1}}\Omega_{t_{L-1}t^{*}}^{\left(L\right)h_{L}}\;.
\end{equation}
In what follows, it is useful to introduce a compact notation for the ``effective input'' to each layer
\begin{equation}
    \xi^{\left(L-\ell\right)h_{L-\ell}\ldots h_{L}}\coloneqq\frac{1}{\sqrt{N_{L-\ell-1}H_{L-\ell-1}}}\sum_{t_{L-\ell}, \ldots,t_{L-1}=1}^Tx_{t_{L-\ell}}^{\left(L-\ell\right)}\Omega_{t_{L-\ell}t_{L-\ell+1}}^{\left(L-\ell\right)h_{L-\ell}}\ldots\Omega_{t_{L-1},t^*}^{\left(L\right)h_{L}}\;,
\end{equation}
$\ell=1,\ldots,L-1$, and for the last attention layer
\begin{equation}
    \xi^{\left(L\right)h_L}\coloneqq\frac{1}{\sqrt{N_{L-1} H_{L-1}}}\sum_{h_{L-1}=1}^{H_{L-1}} V^{(L-1)h_{L-1}}\xi^{(L-1)h_{L-1}h_L}\;.
\end{equation}

\begin{figure}
    \centering
    \hspace{-1em}\includegraphics[width=1.1\textwidth]{illustration.pdf}
    \caption{Schematic representation of the architecture under consideration.}
    \label{fig:illustration}
\end{figure}

\subsection{Posterior distribution}
We are interested in computing the posterior distribution over the network's learnable weights $\Theta\coloneqq\left(V^{\left(0\right)},\left\{ V^{\left(\ell\right)h}\right\} _{\ell,h=1}^{L,H},a\right)$. This is analogous to the Gibbs distribution in statistical physics and is defined as
\begin{equation}
p\left(\Theta\right)=\frac 1 Z \exp\left\{ -\frac{1}{2\mathcal{T}}\sum_{\mu=1}^{P}\left[f\left(x^{\left(0\right)\mu},\Theta\right)-y^{\mu}\right]^{2}-\frac{1}{2\sigma^{2}}\left\Vert \Theta\right\Vert ^{2}\right\} \;,
\end{equation}
where $Z$ indicates the normalization, also called partition function, and $\mathcal{T}$ is the Gibbs temperature. \Fnotes{def Frobenius norm in general} It is useful to introduce a set of auxiliary variables $\{\tt^\mu\}_{\mu=1}^P$ in order to linearize the squared error. The partition function then reads
\begin{align}
   Z\propto \int \dd\Theta\,\dd\tt \,\exp\left(-\frac{\mathcal{T}}{2}\Vert\tt\Vert^2 -\frac{1}{2\sigma^2}\Vert \Theta\Vert^2 +\sum_{\mu=1}^P\ii \tt^\mu\left(f\left(x^{\left(0\right)\mu},\Theta\right)-y^{\mu}\right)\right)\;,
\end{align}
where we have used the symbol $``\propto"$ to indicate that we are neglecting multiplicative constants. We can progressively integrate over all the learnable weights, starting from the readout $a$ and proceeding backwards through the value weights $V^{(\ell)h}$ until the first projection layer $V^{(0)}$. This procedure follows the lines of \citep{li2021statistical,li2022globally}.
\paragraph{Integral over the readout weights ---} We start by computing the integral over the readout weights $a\in\mathbb{R}^{N_{L+1}}$:
\begin{equation}
\begin{split}
    Z\propto\\\int \dd V^{(0)}\left[\prod_{\ell=1}^L\prod_{h_\ell=1}^{H_\ell}\dd V^{(\ell)h_\ell}\right]\dd \tt\exp\left(-\frac{\mathcal{T}}{2}\Vert\tt\Vert^2-\frac{1}{2\sigma^2}\Vert V^{(0)}\Vert^2 -\frac{1}{2\sigma^2}\sum_{\ell=1}^L\sum_{h_\ell=1}^{H_\ell}\Vert V^{(\ell)h_\ell}\Vert^2 \right)\\\times\int \dd a \exp\left(-\frac{1}{2\sigma^2}\Vert a\Vert^2-\sum_{\mu=1}^P\ii \tt^\mu y^\mu +\sum_{\mu=1}^P\ii \tt^\mu\frac{a^\top x_{t^*}^{(L+1),\mu}}{\sqrt{N_{L+1}}}\right)\\
    \propto\int \dd V^{(0)}\left[\prod_{\ell=1}^L\prod_{h_\ell=1}^{H_\ell}\dd V^{(\ell)h_\ell}\right]\dd \tt\exp\left(-\frac{1}{2\sigma^2}\Vert V^{(0)}\Vert^2 -\frac{1}{2\sigma^2}\sum_{\ell=1}^L\sum_{h=1}^{H_\ell}\Vert V^{(\ell)h_\ell}\Vert^2 \right)\\\times
    \exp\left(-\sum_{\mu=1}^P\ii \tt^\mu y^\mu-\frac{\mathcal{T}}{2}\Vert\tt\Vert^2-\frac{\sigma^2}{2 }\sum_{\mu,\nu=1}^P\tt^\mu \tt^\nu\frac{{x_{t^*}^{(L+1),\mu}}^\top x_{t^*}^{(L+1),\nu}}{N_{L+1}} \right)\;.
\end{split}
\end{equation}
\Fnotes{Here I do not think we need to keep track of all multiplicative constants as for the physical interpretation}
Moreover, given that we are interested in the minima of the loss landscape, we can set the Gibbs temperature to zero $\mathcal{T}=0$.
\paragraph{Integral over the value weights at layer $L$ ---} We continue our backward integration starting from the last value weights $V^{(L)}$:
\begin{equation}
\begin{split}
    Z\propto \int \dd V^{(0)}\left[\prod_{\ell=1}^{L-1}\prod_{h_\ell=1}^{H_\ell}\dd V^{(\ell)h_\ell}\right]\dd \tt \exp\left(-\frac{1}{2\sigma^2}\Vert V^{(0)}\Vert^2 -\frac{1}{2\sigma^2}\sum_{\ell=1}^{L-1}\sum_{h_\ell=1}^{H_\ell}\Vert V^{(\ell)h_\ell}\Vert^2 \right)\\\times\exp\left(-\sum_{\mu=1}^P\ii \tt^\mu y^\mu\right)\\\times \int \left[\prod_{h=1}^{H_L}\dd V^{(L)h}\right]\exp\left(-\frac{1}{2\sigma^2}\sum_{h_\ell=1}^{H_L}\Vert V^{(L)h_\ell}\Vert^2\right)\\\times\exp\left(-\frac{\sigma^2}{2}\sum_{\mu,\nu=1}^P \tt^\mu \tt^\nu\frac{\sum_{h_L,\tilde h_L=1}^{H_L}{\xi^{(L)h_L,\mu}}^\top {V^{(L)h_L}}^\top V^{(L)\tilde h_L}\xi^{(L)\tilde h_L, \nu}}{N_{L+1} N_L H_L}\right)\;.
    \end{split}
\end{equation}
The first index in $V^{(L)h_L}$ can be factored out, which leaves us with $N_{L+1}$ identical copies of the integral
\begin{equation}
\begin{split}
    \int\left[ \prod_{h_L=1}^{H_L}\prod_{j=1}^{N_L}\dd V^{(L)h_L}_{1j}\right]\exp\left(-\frac 12 \sum_{h_L,\tilde h_L=1}^{H_L}\sum_{i,j=1}^{N_L}V^{(L)h_L}_{1i}\left[\frac{\delta_{ij}\delta_{h_L \tilde h_L}}{\sigma^2}+v_i^{h_L}v_j^{\tilde h_L}\right]V_{1j}^{(L)\tilde h_L}\right)\\\propto
    \frac{1}{\sqrt{\det\left(\text{Id}+\sigma^2 vv^\top\right)}}
    \end{split}
\end{equation}
\Fnotes{Here I use the most simplified notation where again all constants go in the $``\propto''$}
where we define
\begin{equation}
    v_i^{h_L}\coloneqq\sqrt{\frac{\sigma^4}{N_{L+1}N_LH_L}}\sum_{\mu=1}^P\tt^\mu \xi_i^{(L)h_L,\mu}\;,
\end{equation}
and we denote by $v$ the vector whose indices run over the pair $(i,h_L)$. Applying the matrix determinant lemma: $\det\left(\text{Id}+\sigma^2 vv^\top\right)=1+\sigma^2 v^\top v$, we find
\begin{equation}
\begin{split}
    Z\propto\int \dd V^{(0)}\left[\prod_{\ell=1}^{L-1}\prod_{h_\ell=1}^{H_\ell}\dd V^{(\ell)h_\ell}\right]\dd \tt \exp\left(-\frac{1}{2\sigma^2}\Vert V^{(0)}\Vert^2 -\frac{1}{2\sigma^2}\sum_{\ell=1}^{L-1}\sum_{h_\ell=1}^{H_\ell}\Vert V^{(\ell)h_\ell}\Vert^2 \right)\\\times\exp\left(-\sum_{\mu=1}^P\ii \tt^\mu y^\mu-\frac{N_{L+1}}{2}\log\left(1+\frac{\sigma^2}{N_{L+1}}\sum_{\mu,\nu=1}^P\tt^\mu \tt^\nu C^{(L+1),\mu\nu}\right)\right)\;,
\end{split}
\end{equation}
where we have defined the \emph{pre-kernel} $C^{(L+1),\mu\nu}$ as
\begin{equation}
    C^{(L+1),\mu\nu}\coloneqq \frac{\sigma^2}{N_L H_L}\sum_{h_L=1}^{H_L}{\xi^{(L)h_L,\mu}}^\top \xi^{(L)h_L,\nu}\;.
\end{equation}
\paragraph{Order parameter at layer $L$ ---} We introduce the definition of the following order parameter
\begin{equation}
    H^{(L+1)}\coloneqq \frac{\sigma^2}{N_{L+1}}\sum_{\mu,\nu=1}^P\tt^\mu \tt^\nu C^{(L+1),\mu\nu}\;,
\end{equation}
and its Fourier conjugate $U^{(L+1)}$. The partition function can be written as 
\begin{equation}
\begin{split}
 Z   \propto \int \dd H^{(L+1)}\,\dd U^{(L+1)}\,\dd \tt\, \dd V^{(0)}\exp\left(-\sum_{\mu=1}^P\ii \tt^\mu y^\mu+\frac{N_{L+1}}{2\sigma^2}H^{(L+1)} U^{(L+1)}\right)\\\times\exp\left(-\frac{N_{L+1}}{2}\log\left(1+H^{(L+1)}\right)-\frac{1}{2\sigma^2}\Vert V^{(0)}\Vert^2\right)\\\times\int \left[\prod_{\ell=1}^{L-1}\prod_{h_\ell=1}^{H_\ell}\dd V^{(\ell)h_\ell}\right]\exp\left(-\frac{1}{2\sigma^2}\sum_{\ell=1}^{L-1}\sum_{h_\ell=1}^{H_\ell}\Vert V^{(\ell)h_\ell}\Vert^2-\frac{1}2 U^{L+1}\sum_{\mu,\nu}\tt^\mu \tt^\nu C^{(L+1),\mu\nu}\right)\;.
 \end{split}
\end{equation}
\paragraph{Integral over the value weights at layer $(L-1)$ ---}


\section{Physical interpretation of the order parameter}
\begin{figure}[ht!]
    \centering
    \includegraphics[width=1\textwidth]{draft.pdf}
    \caption{Caption}
    \label{fig:enter-label}
\end{figure}

